EXMODD: An EXplanatory Multimodal Open-Domain Dialogue dataset

The need for high-quality data has been a key issue hindering the research of dialogue tasks. Recent studies try to build datasets through manual, web crawling, and large pre-trained models. However, man-made data is expensive and data collected from the internet often includes generic responses, meaningless statements, and toxic dialogues. Automatic data generation through large models is a cost-effective method, but for open-domain multimodal dialogue tasks, there are still three drawbacks: 1) There is currently no open-source large model that can accept multimodal input; 2) The content generated by the model lacks interpretability; 3) The generated data is usually difficult to quality control and require extensive resource to collect. To alleviate the significant human and resource expenditure in data collection, we propose a Multimodal Data Construction Framework (MDCF). MDCF designs proper prompts to spur the large-scale pre-trained language model to generate well-formed and satisfactory content. Additionally, MDCF also automatically provides explanation for a given image and its corresponding dialogue, which can provide a certain degree of interpretability and facilitate manual follow-up quality inspection. Based on this, we release an Explanatory Multimodal Open-Domain dialogue dataset (EXMODD). Experiments indicate a positive correlation between the model's ability to generate accurate understandings and high-quality responses. Our code and data can be found at https://github.com/poplpr/EXMODD.

==> addition.tex <==
\begin{table*}
\centering
\begin{tabular}{lcccc}
\hline
\textbf{Dataset} & \textbf{coherence} & \textbf{distinct-1} & \textbf{distinct-2} & \textbf{distinct-3} \\
\hline
VisDial \cite{Das_2017_CVPR} & 63.60 & 1.03 & 12.62 & 36.61 \\
IGC \cite{guo-etal-2017-ijcnlp} & 81.02 & 16.09 & 49.40 & 75.12 \\
DialyDialog \cite{li-etal-2017-dailydialog} & 82.32 & 2.05 & 20.31 & 51.20 \\
OpenSubtitles \cite{lison-tiedemann-2016-opensubtitles2016} & 80.85 & 0.77 & 10.08 & 31.23 \\
\hline
Image-Chat \cite{shuster-etal-2020-image} & 79.14 & 5.69 & 36.09 & 72.54 \\
Image-Chat Context \cite{shuster-etal-2020-image} & - & 6.13 & 37.10 & 72.07 \\
\hline
EXMODO & 81.59 & 9.43 & 42.19 & 72.04 \\
\hline
\end{tabular}
\caption{\label{dataset metrics}
Distinct-1,2,3, coherence of datasets.
}
\end{table*}


% Toxity table
\begin{table} \small
\centering
\begin{tabular}{lc}
\hline
\textbf{Dataset} & \textbf{Toxity}  \\
\hline
VisDial \cite{Das_2017_CVPR} & 1.28 \\
IGC \cite{guo-etal-2017-ijcnlp} & 1.27 \\
DialyDialog \cite{li-etal-2017-dailydialog} & 1.44 \\
OpenSubtitles \cite{lison-tiedemann-2016-opensubtitles2016} & 8.21 \\
\hline
Image-Chat \cite{shuster-etal-2020-image} & 5.41 \\
Image-Chat Context \cite{shuster-etal-2020-image} & 5.08 \\
\hline
EXMODO & \textbf{0.52} \\
\hline
\end{tabular}
\caption{\label{Toxity}
The toxic bert score of EXMODO and other dataset response.
}
\end{table}
